ADW: Blockchain-enabled Small-scale Farm Digitization

Farm records hold the static, temporal, and longitudinal details of the farms. For small-scale farming, the ability to accurately capture these records plays a critical role in formalizing and digitizing the agriculture industry. Reliable exchange of these record through a trusted platform could unlock critical and valuable insights to different stakeholders across the value chain in agriculture eco-system. Lately, there has been increasing attention on digitization of small scale farming with the objective of providing farm-level transparency, accountability, visibility, access to farm loans, etc. using these farm records. However, most solutions proposed so far have the shortcoming of providing detailed, reliable and trusted small-scale farm digitization information in real time. To address these challenges, we present a system, called Agribusiness Digital Wallet (ADW), which leverages blockchain to formalize the interactions and enable seamless data flow in small-scale farming ecosystem. Utilizing instrumentation of farm tractors, we demonstrate the ability to utilize farm activities to create trusted electronic field records (EFR) with automated valuable insights. Using ADW, we processed several thousands of small-scale farm-level activity events for which we also performed automated farm boundary detection of a number of farms in different geographies.

==> sections/background.tex <==
\section{Background and Motivation}
%\textcolor{red}{This section needs more love. Let us improve it - we need to make a strong case. We need a clean business process diagram!}

\begin{comment}
\subsection{Background and Motivation}
\label{sec:background}

Cooperative networks (and hence small-scale farmers) across all the agriculture value chains use very limited data and rely on their experience and intuitions to determine when making farming decisions.  Where the data exists, the unverified sources, fragmented and unrepresentative nature of the data sets lead to unreliable decisions. Moreover, they rely on manual processes due to the largely non-digitized nature of the industry. In the rare cases where there is a decisioning platform, it only covers a very small part of the value chain and often times critical datasets are not captured. 
This creates bottlenecks for many participants in the small-scale agriculture ecosystem such as aggregator companies, input companies, financial institutions, logistics companies, development partners, all of whom need trusted and verifiable data sources and analytics solutions to make critical decisions.
%such as resource allocation. 
For example, banks and financial institutions continue to struggle to understand  data value chains despite their desire to open up wide-range of agriculture finance services (e.g., credit, loan, insurance, and underwriting) for these classes of farmers (small-scale and medium-scale farmers) and mechanization/tractor service providers. Ultimately, this significantly delays otherwise hinders informative decisions for the growth and productivity of the small-scale farming ecosystem.
%in emerging market countries where their economies are tightly coupled with agriculture and dominated by small-scale farming.  

There have been many efforts to address some of the above challenges which include the introduction of \say{Uber-like} tractor services, by agri-based start-up named Hello Tractor (HT)\cite{ht}. HT introduced a mobile platform enables farmers to request for tractors services from their phones. 
HT enables interactions between farmers and tractor service providers via their \emph{Booking} app, \emph{Scheduling} app, and \emph{Monitoring} devices.
For example, a farmer that wishes to request a tractor service will contact an extension officer (typically a trained agronomist who work as \say{service agent}) allocated to his/her region. The extension officer would then visit the farmer and collect survey information about the farm. This involves walking around the boundary of the farm while recording the geo-coordinates using HT's booking application. Along with the boundary information, the extension worker also records the primary and secondary crop, tractor service type and some contextual data about the farmer and the farm. This request is termed as a \emph{Service-Booking} within the HT platform and is forwarded to the \emph{Scheduling} app, which is used by the tractor fleet managers to aid them in fleet and resource management. However, due to the involvement of multiple actors in the data value chain, there is no way to verify the authenticity of the data.
 

To effectively utilize a tractor, fleet managers define a minimum threshold that is the acreage that must be satisfied before deploying a tractor to the field. This essentially means that a tractor will be deployed to work on a given booking or set of bookings if it satisfies the minimum acreage defined and availability of a tractor is confirmed. Finally, fleet owners need to relay the utilization (measure of profitability) of their fleet to their finical institutes for affordable banking services (e.g., borrowing).  However,  trust (as a result of lack of end-to-end visibility) continued to be one of the major issues among these entities due to the nature of interactions among these parties and the data value chain. Because of this trust issue today most of the fleet/tractor owners are subject to high interest rates (often 100\% collateral) in developing countries.

One effort aimed at creating and developing digital twins or virtual models of the world’s farms is the Electronic Field Record (EFR), a concept analogous to that commonly known in the medical domain for patient data – EMR for Electronic Medical Records. The promise of the EFR is to keep track every ‘moment of truth’ about farms, from events on a farm such as soil analysis results, soil moisture levels, planted crops, detected or predicted crop diseases, crop yields, to possible interactions with the farm such as history of cultivations, fertilizers being used, soil treatment methods being followed, pesticides being used. EFRs will become the basis of information sharing by providing timestamped ‘moments of truth’ about farmlands. 
\end{comment}

\begin{comment}

\textcolor{blue}{ Kommy and Regi to finalize on this section }

\iffalse
\textcolor{red}{Note: will call out the specific challenges that triggers the need for food supply chains to modernize in terms of digitization, information sharing, and making multi-party transactions more efficient, using technologies including blockchain and we will provide examples and references of developments across the industry: } 
\fi

Generally, we can all agree that the way agriculture is currently done could benefit from modernization from how farm inputs are chosen, acquired and used to how harvests are collected and distributed. However, how modernization is done will different wildly between large-scale farming operations and small-holder distributed farming networks. While the former benefits from legacy systems which becomes a feat of engineering in order to harmonize those systems into interoperable ditigal systems. Digitizing small-holder distributed farming networks becomes a much more challenging task. Simply knowing and tracking millions of farm boundaries is a daunting task even if satellite imagery and ground-level paper-based date registries are used.



\textcolor{blue}{Local Small-Holder Example}

\textcolor{blue}{Global Small-Holder Example}

Mars push for sustainable chocolate production in the face of deforestation and child labour in Ghana and the Ivory Coast. Such issues are tractable and requires the hamonization of satellite and ground-level, scalable surveys in order to detect increasing farm boundaries and properly certify the portion of millions of distibuted farmers who are adhering to sustainable farming practices\cite{chocolate_mufson}.

%\cite{chocolate_mufson}

\textcolor{red}{ Block model Farming approach which motivates our focus}


\textcolor{red}{ Uber-tractor business model}

One effort aimed at creating and developing digital twins or virtual models of the world’s farms is the Electronic Field Record (EFR), a concept analogous to that commonly known in the medical domain for patient data – EMR for Electronic Medical Records. The promise of the EFR is to keep track every ‘moment of truth’ about farms, from events on a farm such as soil analysis results, soil moisture levels, planted crops, detected or predicted crop diseases, crop yields, to possible interactions with the farm such as history of cultivations, fertilizers being used, soil treatment methods being followed, pesticides being used. EFRs will become the basis of information sharing by providing timestamped ‘moments of truth’ about farmlands. Hello Tractor \cite{ht} is a mobile platform that enables farmers to access tractor services on demand, and is already benefiting from EFR by providing credit scores for loans for small-scale farmers who typically have no access to banks, by utilizing historical timestamped data about their farms.

We believe that blockchain offers a standards based information sharing platform. In the agriculture domain there are already successful examples of large private corporations either trialling or mandating that their consumers will be able to scan codes on packaged products and be able to trace the travel of the foodstuff in their hand from its source in a farm, all through the supply chain, to its destination in a shop shelf (colloquially called farm-to-fork). One examples is IBM Food Trust [20] which is a solution targeted at sharing certification and enabling traceability of food products being used by Walmart and other retailers.

Efforts to streamline financial transactions in agricultural ecosystems are also underway. Private sector examples in the trading space include LDC and ING [17] partnering to trial on soybean trade platform and the ADM, Bunge, Cargill, Louis Dreyfuss consortium considering wider efficiencies in global agricultural commodity trades [18]. Additional use cases include technology platforms that have been developed to establish digital marketplaces for agricultural inputs and direct-to-consumer access for growers.
\end{comment}

